An unfitted discontinuous Galerkin scheme for conservation laws on evolving surfaces

Motivated by considering partial differential equations arising from conservation laws posed on evolving surfaces, a new numerical method for an advection problem is developed and simple numerical tests are performed. The method is based on an unfitted discontinuous Galerkin approach where the surface is not explicitly tracked by the mesh which means the method is extremely flexible with respect to geometry. Furthermore, the discontinuous Galerkin approach is well-suited to capture the advection driven by the evolution of the surface without the need for a space-time formulation, back-tracking trajectories or streamline diffusion. The method is illustrated by a one-dimensional example and numerical results are presented that show good convergence properties for a simple test problem.

==> extra_packages/cleveref/README <==
cleveref, a LaTeX package for intelligent cross-referencing
Copyright (C) 2007--2013  Toby Cubitt

Files:
cleveref.ins  Batch file, run through LaTeX
cleveref.dtx  Docstrip archive, run through LaTeX
cleveref.sty  LaTeX package, generated by cleveref.ins from cleveref.dtx
cleveref.dvi  Package documentation, generated from cleveref.dtx
cleveref.pdf  Package documentation; can also be generated from cleveref.dtx
README        This file

E-mail:   toby-cleveref@dr-qubit.org
Address:  DAMTP, University of Cambridge, United Kingdom

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


Description:
------------
The cleveref package enhances LaTeX's cross-referencing features, allowing the
format of cross-references to be determined automatically according to the
"type" of cross-reference (equation, section, etc.) and the context in which
the cross-reference is used. The formatting for each cross-reference type can
be fully customised in the preamble of your document. In addition, cleveref
can type-set cross-references to lists of multiple labels, automatically
formatting them according to their types, sorting them, and compressing
sequences of numerically consecutive labels. Again, the multiple-reference
formatting is fully customisable. Though a number of other packages provide
similar features, all have certain deficiencies which cleveref attempts to
overcome.

Using cleveref is easy. Basically, wherever you would previously have used
\ref, you can use \cref instead. (Except at the beginning of a sentence, where
you should use \Cref.)  You no longer need to put the name of the thing you're
referencing in front of the \cref command, because cleveref will sort that out
for you: i.e. use "\cref{eq1}" instead of "eq.~(\ref{eq1})". If you want to
refer to a range of labels, use the \crefrange command: "\crefrange{eq1}{eq5}"
produces "eqs.~(1) to~(5)". Finally, if you want to refer to multiple things
at once, you can now combine them all into one cross-reference and leave
cleveref to sort it out: e.g. "\cref{eq2,eq1,eq3,eq5,thm2,def1}" produces:
"eqs.~(1) to~(3) and~(5), theorem~5, and definition~1".

Cleveref has various other useful features. For details, see the package
documentation.


==> extra_packages/ntheorem/README <==
ntheorem.dtx includes the style-file, a standard configuration, and the
documentation.  Additional information (including a test-file) is
available at

    http://user.informatik.uni-goettingen.de/~may/Ntheorem/

We recommend placing the unpacked files (and this message) in an extra
directory

    macros/latex/contrib/ntheorem/

Wolfgang May & Andreas Schedler

--------------------

Abstract:

ntheorem.sty for LaTeX

by Wolfgang May and Andreas Schedler

ntheorem.sty is a package for handling theorem-like environments.
Aditionally to several features for defining the layout of
theorem-like environments which can be regarded to be standard
requirements for a theorem-package, it provides solutions for two
related problems:  placement of endmarks and generation of lists
of theorem-like environments.

In contrast to former approaches, it solves the problem of
setting endmarks of theorem-like environments (theorems,
definitions, examples, and proofs) automatically at the right
positions, even if the environment ends with a displaymath or
(even nested) list environments, it also copes with the amsmath
package.  This is done in the same manner as the handling of
labels by using the .aux file.

It also introduces the generation of lists of theorem-like
environments in the same manner as listoffigures. Additionally,
more comfortable referencing is supported.

After running LaTeX several times (depending on the complexity of
references, in general, three runs are sufficient), the endmarks
are set correctly, and theoremlists are generated.

Since ntheorem.sty uses the standard LaTeX \newtheorem command,
existing documents can be switched to ntheorem.sty without having
to change the .tex file.  Also, it is compatible with LaTeX files
using theorem.sty written by Frank Mittelbach.

Features:

 * General Layout of Theorems:
   different predefined theoremstyles, according to theorem.sty,
   defining own theoremstyles by \newtheoremstyle,
 * Placement of End Marks:
   automatically setting end marks for theorem-like environments
   in text, math environments, lists etc.,
 * Generation of Theorem Lists:
   Generation of list-of-theorem similar to list-of-figures,
   different predefined liststyles, according to theorem.sty,
   defining own liststyles by \newliststyle,
 * Referencing:
   Extended referencing feature, yielding, e.g. "Theorem 42".


==> extra_packages/siamart/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{An Example Article} 
\newcommand{\TheAuthors}{D. Doe, P. T. Frank, and J. E. Smith}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}

% Authors: full names plus addresses.
\author{
  Dianne Doe\thanks{Imagination Corp., Chicago, IL
    (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
  \and
  Paul T. Frank\thanks{Department of Applied Mathematics, Fictional
    University, Boise, ID (\email{ptfrank@fictional.edu},
    \email{jesmith@fictional.edu}).}
  \and
  Jane E. Smith\footnotemark[3]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

